Comparing the costs of abstraction for DL frameworks

High level abstractions for implementing, training, and testing Deep Learning (DL) models abound. Such frameworks function primarily by abstracting away the implementation details of arbitrary neural architectures, thereby enabling researchers and engineers to focus on design. In principle, such frameworks could be "zero-cost abstractions"; in practice, they incur translation and indirection overheads. We study at which points exactly in the engineering life-cycle of a DL model the highest costs are paid and whether they can be mitigated. We train, test, and evaluate a representative DL model using PyTorch, LibTorch, TorchScript, and cuDNN on representative datasets, comparing accuracy, execution time and memory efficiency.

==> figures/stack_traces/stacks.tex <==
\begin{figure*}[h]
  \centering
  \begin{adjustbox}{width=\textwidth}
    \centering
    \begin{tikzpicture}[scale=.8]

      \tikzstyle{padding}=[fill=red!10,draw=red!50!black]
      \tikzstyle{freecell}=[fill=red!10,draw=red!30!black]
%      \tikzstyle{freestruct}=[fill=blue!10,draw=blue!30!black]

      \stacktop{}
      \cell{\scriptsize\texttt{call\_function}} \coordinate (p3) at (currentcell.east);
      \startframe
      \padding{2}{\large\vdots}
      \finishframe{30 calls\hspace*{0.3cm}}
      \cell[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\scriptsize\texttt{at::conv2d}}               \coordinate (p2) at (currentcell.east);
      \startframe
      \llcell{3}{pattern=north west lines, pattern color=green!50, draw=green!50!black}{\large\vdots}
%      \padding{3}{\large\vdots}
      \finishframe{61 calls\hspace*{0.3cm}}
      \cell[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\scriptsize\texttt{cudnnConvolutionForward}}
      \cell[draw=none]{PyTorch call stack}

      \draw[freecell] (5,-1)
      +(-2,.5) -- +(-2,-.5) -- +(2,-.5) -- +(2,.5);
      \draw (5,-1+1/6) node{\vdots};
      \drawstruct{(5,-1)})
      \structcell[freecell]{\scriptsize\texttt{Conv2dImpl::forward}}
      \structcell[freecell]{\scriptsize\texttt{functional::detail::conv2d}}
      \structcell[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\scriptsize\texttt{at::conv2d}}
      \structcellpaddingthree[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\vdots}
      \structcell[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\scriptsize\texttt{cudnnConvolutionForward}}
      \structcell[draw=none]{LibTorch call stack}

      \draw[freecell] (10,-6)
      +(-2,.5) -- +(-2,-.5) -- +(2,-.5) -- +(2,.5);
      \draw (10,-6+1/6) node{\vdots};
      \drawstruct{(10,-6)}
      \structcell[freecell]{\scriptsize\texttt{Conv2d<float>::forward}}
      \structcell[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\scriptsize\texttt{cudnnConvolutionForward}}
      \structcell[draw=none]{cuDNN call stack}

      \draw[freecell] (15,-4)
      +(-2,.5) -- +(-2,-.5) -- +(2,-.5) -- +(2,.5);
      \draw (15,-4+1/6) node{\vdots};
      \drawstruct{(15,-4)}
      \structcell[freecell]{\tiny\texttt{autograd::VariableType::\_convolution}}
      \structcellpadding[freecell]{\vdots}
      \structcell[pattern=north west lines, pattern color=green!50, draw=green!50!black]{\scriptsize\texttt{cudnnConvolutionForward}}
      \structcell[draw=none]{TorchScript call stack}
      \draw[snake=brace, line width=0.6pt, segment amplitude=7pt]
      (17,-5-0.5) -- (17,-7-0.5) node [black,midway,xshift=1cm] {14 calls};

    \end{tikzpicture}
  \end{adjustbox}
  \caption["Short" caption without tikz code]{Call stacks representing the number of calls between \code{Conv2d.forward} at the level of abstraction and the ultimate execution of the convolution \code{cudnnConvolutionForward} on the GPU. \tikz{\path[fill=red!10,draw=red!50!black] (0,0) rectangle (.25cm,.25cm);} represents calls where the implementations diverge and \tikz{\path[pattern=north west lines, pattern color=green!50, draw=green!50!black] (0,0) rectangle (.25cm,.25cm);} represents calls where the implementations coincide. Note that program setup calls are omitted. These were produced by building each implementation with debug symbols and using \code{gdb} to set a breakpoint at \code{cudnnConvolutionForward}. Complete stacktraces are available on GitHub at \link{\href{https://github.com/makslevental/pytorch_abstraction_comparison/tree/main/tex/stack_traces}{main/tex/stack\_traces}}.}
  \label{fig:stacks}
\end{figure*}

